Photometric Completeness Modelled With Neural Networks

In almost any study involving optical/NIR photometry, understanding the completeness of detection and recovery is an essential part of the work. The recovery fraction is, in general, a function of several variables including magnitude, color, background sky noise, and crowding. We explore how completeness can be modelled, {with the use of artificial-star tests,} in a way that includes all of these parameters \emph{simultaneously} within a neural network (NN) framework. The method is able to manage common issues including asymmetric completeness functions and the bilinear dependence of the detection limit on color index. We test the method with two sample HST (Hubble Space Telescope) datasets: the first involves photometry of the star cluster population around the giant Perseus galaxy NGC 1275, and the second involves the halo-star population in the nearby elliptical galaxy NGC 3377. The NN-based method achieves a classification accuracy of $>$\,94\%, and produces results entirely consistent with more traditional techniques for determining completeness. Additional advantages of the method are that none of the issues arising from binning of the data are present, and that a recovery probability can be assigned to every individual star in the real photometry. Our data, models, and code (called COINTOSS) can be found online on Zenodo at the following link: https://doi.org/10.5281/zenodo.8306488.

==> alldata.tex <==
% latex table generated in R 3.6.1 by xtable 1.8-4 package
% Fri Dec  4 13:30:41 2020
\begin{table}[ht]
\centering
\begin{tabular}{rrrrrrlrl}
  \hline
 & log10Mstar & Type & hasGC & Ngc & logMgc & Name & logMh & Sample \\ 
  \hline
2 & 4.85 & -3.00 &   1 & 1.00 & 3.60 & EriII & 8.24 & Local Group Sample \\ 
  3 & 6.37 & 9.90 &   1 & 1.00 & 4.16 & Aquarius & 9.29 & Local Group Sample \\ 
  4 & 6.01 & -3.00 &   1 & 1.00 & 4.18 & AndXXV & 9.06 & Local Group Sample \\ 
  5 & 7.01 & 9.80 &   1 & 1.00 & 5.06 & PegdIrr & 9.76 & Local Group Sample \\ 
  6 & 8.65 & 8.90 &   1 & 1.00 & 5.51 & SMC & 10.90 & Local Group Sample \\ 
  7 & 7.81 & 9.90 &   1 & 1.00 & 5.70 & WLM & 10.35 & Local Group Sample \\ 
  8 & 8.13 & 9.90 &   1 & 1.00 & 5.74 & IC10 & 10.58 & Local Group Sample \\ 
  9 & 8.05 & -4.80 &   1 & 8.00 & 5.83 & NGC185 & 10.52 & Local Group Sample \\ 
  10 & 7.49 & -4.80 &   1 & 5.00 & 5.86 & Fornax & 10.12 & Local Group Sample \\ 
  11 & 8.21 & 9.80 &   1 & 8.00 & 6.10 & NGC6822 & 10.64 & Local Group Sample \\ 
  12 & 7.97 & -4.70 &   1 & 10.00 & 6.11 & NGC147 & 10.47 & Local Group Sample \\ 
  13 & 8.73 & -4.80 &   1 & 11.00 & 6.15 & NGC205 & 10.93 & Local Group Sample \\ 
  14 & 7.89 & -3.00 &   1 & 11.00 & 6.15 & GaiaEnc & 10.41 & Local Group Sample \\ 
  15 & 7.53 & -3.00 &   1 & 8.00 & 6.44 & Sgr & 10.31 & Local Group Sample \\ 
  16 & 9.17 & 9.10 &   1 & 16.00 & 6.52 & LMC & 11.14 & Local Group Sample \\ 
  17 & 9.53 & 5.90 &   1 & 50.00 & 6.70 & M33 & 11.31 & Local Group Sample \\ 
  18 & 10.72 & 4.00 &   1 & 160.00 & 7.20 & MilkyWay & 12.70 & Local Group Sample \\ 
  19 & 10.92 & 3.00 &   1 & 450.00 & 7.65 & M31 & 13.42 & Local Group Sample \\ 
  20 & 5.74 & -4.90 &   0 & 0.00 & 0.00 & UrsaMinor &  & Local Group Sample \\ 
  21 & 2.33 & -3.00 &   0 & 0.00 & 0.00 & VirgoI &  & Local Group Sample \\ 
  22 & 3.17 & -3.00 &   0 & 0.00 & 0.00 & Willman1 &  & Local Group Sample \\ 
  23 & 7.17 & -4.00 &   0 & 0.00 & 0.00 & AndVII &  & Local Group Sample \\ 
  24 & 5.17 & -3.00 &   0 & 0.00 & 0.00 & AndX &  & Local Group Sample \\ 
  25 & 4.89 & -3.00 &   0 & 0.00 & 0.00 & AndXI &  & Local Group Sample \\ 
  26 & 4.69 & -3.00 &   0 & 0.00 & 0.00 & AndXII &  & Local Group Sample \\ 
  27 & 4.81 & -3.00 &   0 & 0.00 & 0.00 & AndXIII &  & Local Group Sample \\ 
  28 & 5.49 & -3.00 &   0 & 0.00 & 0.00 & AndXIV &  & Local Group Sample \\ 
  29 & 5.81 & -3.00 &   0 & 0.00 & 0.00 & AndXIX &  & Local Group Sample \\ 
  30 & 5.89 & -3.00 &   0 & 0.00 & 0.00 & AndXV &  & Local Group Sample \\ 
  31 & 5.81 & -3.00 &   0 & 0.00 & 0.00 & AndXVI &  & Local Group Sample \\ 
  32 & 5.61 & -3.00 &   0 & 0.00 & 0.00 & AndXVII &  & Local Group Sample \\ 
  33 & 6.01 & -3.00 &   0 & 0.00 & 0.00 & AndXVIII &  & Local Group Sample \\ 
  34 & 4.65 & -3.00 &   0 & 0.00 & 0.00 & AndXX &  & Local Group Sample \\ 
  35 & 6.09 & -3.00 &   0 & 0.00 & 0.00 & AndXXI &  & Local Group Sample \\ 
  36 & 4.73 & -3.00 &   0 & 0.00 & 0.00 & AndXXII &  & Local Group Sample \\ 
  37 & 6.21 & -3.00 &   0 & 0.00 & 0.00 & AndXXIII &  & Local Group Sample \\ 
  38 & 5.17 & -3.00 &   0 & 0.00 & 0.00 & AndXXIV &  & Local Group Sample \\ 
  39 & 5.45 & -3.00 &   0 & 0.00 & 0.00 & AndXXIX &  & Local Group Sample \\ 
  40 & 4.97 & -3.00 &   0 & 0.00 & 0.00 & AndXXVI &  & Local Group Sample \\ 
  41 & 5.29 & -3.00 &   0 & 0.00 & 0.00 & AndXXVII &  & Local Group Sample \\ 
  42 & 5.53 & -3.00 &   0 & 0.00 & 0.00 & AndXXVIII &  & Local Group Sample \\ 
  43 & 5.62 & -3.00 &   0 & 0.00 & 0.00 & AntliaII &  & Local Group Sample \\ 
  44 & 3.76 & -3.00 &   0 & 0.00 & 0.00 & AquariusII &  & Local Group Sample \\ 
  45 & 4.42 & -3.00 &   0 & 0.00 & 0.00 & BootesI &  & Local Group Sample \\ 
  46 & 3.19 & -3.00 &   0 & 0.00 & 0.00 & BootesII &  & Local Group Sample \\ 
  47 & 4.31 & -3.00 &   0 & 0.00 & 0.00 & BootesIII &  & Local Group Sample \\ 
  48 & 3.82 & -3.00 &   0 & 0.00 & 0.00 & BootesIV &  & Local Group Sample \\ 
  49 & 5.90 & -4.80 &   0 & 0.00 & 0.00 & Carina &  & Local Group Sample \\ 
  50 & 3.81 & -3.00 &   0 & 0.00 & 0.00 & CarinaII &  & Local Group Sample \\ 
  51 & 2.97 & -3.00 &   0 & 0.00 & 0.00 & CarinaIII &  & Local Group Sample \\ 
  52 & 4.23 & -3.00 &   0 & 0.00 & 0.00 & CentaurusI &  & Local Group Sample \\ 
  53 & 6.61 & 10.00 &   0 & 0.00 & 0.00 & Cetus &  & Local Group Sample \\ 
  54 & 2.00 & -3.00 &   0 & 0.00 & 0.00 & CetusII &  & Local Group Sample \\ 
  55 & 2.99 & -3.00 &   0 & 0.00 & 0.00 & CetusIII &  & Local Group Sample \\ 
  56 & 3.79 & -3.00 &   0 & 0.00 & 0.00 & ColumbaI &  & Local Group Sample \\ 
  57 & 3.88 & -3.00 &   0 & 0.00 & 0.00 & ComaBer &  & Local Group Sample \\ 
  58 & 5.29 & -3.00 &   0 & 0.00 & 0.00 & CraterII &  & Local Group Sample \\ 
  59 & 5.50 & -3.00 &   0 & 0.00 & 0.00 & CVnI &  & Local Group Sample \\ 
  60 & 4.08 & -3.00 &   0 & 0.00 & 0.00 & CVnII &  & Local Group Sample \\ 
  61 & 5.65 & -4.80 &   0 & 0.00 & 0.00 & Draco &  & Local Group Sample \\ 
  62 & 3.40 & -3.00 &   0 & 0.00 & 0.00 & GrusI &  & Local Group Sample \\ 
  63 & 3.57 & -3.00 &   0 & 0.00 & 0.00 & GrusII &  & Local Group Sample \\ 
  64 & 4.34 & -3.00 &   0 & 0.00 & 0.00 & Hercules &  & Local Group Sample \\ 
  65 & 3.52 & -3.00 &   0 & 0.00 & 0.00 & Horologium &  & Local Group Sample \\ 
  66 & 7.09 & 10.00 &   0 & 0.00 & 0.00 & AndII &  & Local Group Sample \\ 
  67 & 2.64 & -3.00 &   0 & 0.00 & 0.00 & Horologium &  & Local Group Sample \\ 
  68 & 3.96 & -3.00 &   0 & 0.00 & 0.00 & HydraII &  & Local Group Sample \\ 
  69 & 3.90 & -3.00 &   0 & 0.00 & 0.00 & HydrusI &  & Local Group Sample \\ 
  70 & 8.21 & 9.90 &   0 & 0.00 & 0.00 & IC1613 &  & Local Group Sample \\ 
  71 & 6.97 & 9.90 &   0 & 0.00 & 0.00 & LeoA &  & Local Group Sample \\ 
  72 & 6.84 & -4.70 &   0 & 0.00 & 0.00 & LeoI &  & Local Group Sample \\ 
  73 & 6.03 & 4.80 &   0 & 0.00 & 0.00 & LeoII &  & Local Group Sample \\ 
  74 & 4.01 & -3.00 &   0 & 0.00 & 0.00 & LeoIV &  & Local Group Sample \\ 
  75 & 6.13 & 10.00 &   0 & 0.00 & 0.00 & AndIII &  & Local Group Sample \\ 
  76 & 3.73 & -3.00 &   0 & 0.00 & 0.00 & LeoV &  & Local Group Sample \\ 
  77 & 5.21 & 0.00 &   0 & 0.00 & 0.00 & LeoT &  & Local Group Sample \\ 
  78 & 6.17 & -1.00 &   0 & 0.00 & 0.00 & LGS3 &  & Local Group Sample \\ 
  79 & 5.37 & -3.00 &   0 & 0.00 & 0.00 & AndIX &  & Local Group Sample \\ 
  80 & 3.65 & -3.00 &   0 & 0.00 & 0.00 & PegasusIII &  & Local Group Sample \\ 
  81 & 6.09 & 9.50 &   0 & 0.00 & 0.00 & Phoenix &  & Local Group Sample \\ 
  82 & 3.09 & -3.00 &   0 & 0.00 & 0.00 & PhoenixII &  & Local Group Sample \\ 
  83 & 3.48 & -3.00 &   0 & 0.00 & 0.00 & PictorII &  & Local Group Sample \\ 
  84 & 3.70 & -3.00 &   0 & 0.00 & 0.00 & PiscesII &  & Local Group Sample \\ 
  85 & 3.61 & -3.00 &   0 & 0.00 & 0.00 & ReticulumI &  & Local Group Sample \\ 
  86 & 3.33 & -3.00 &   0 & 0.00 & 0.00 & ReticulumI &  & Local Group Sample \\ 
  87 & 6.46 & -4.80 &   0 & 0.00 & 0.00 & Sculptor &  & Local Group Sample \\ 
  88 & 2.53 & -3.00 &   0 & 0.00 & 0.00 & SegueI &  & Local Group Sample \\ 
  89 & 5.77 & -3.00 &   0 & 0.00 & 0.00 & AndV &  & Local Group Sample \\ 
  90 & 2.80 & -3.00 &   0 & 0.00 & 0.00 & SegueII &  & Local Group Sample \\ 
  91 & 5.59 & -3.00 &   0 & 0.00 & 0.00 & SextansI &  & Local Group Sample \\ 
  92 & 6.73 & 10.00 &   0 & 0.00 & 0.00 & SgrdIrr &  & Local Group Sample \\ 
  93 & 2.65 & -3.00 &   0 & 0.00 & 0.00 & Triangulum &  & Local Group Sample \\ 
  94 & 5.93 & -4.90 &   0 & 0.00 & 0.00 & Tucana &  & Local Group Sample \\ 
  95 & 3.57 & -3.00 &   0 & 0.00 & 0.00 & TucanaII &  & Local Group Sample \\ 
  96 & 3.34 & -3.00 &   0 & 0.00 & 0.00 & TucanaIV &  & Local Group Sample \\ 
  97 & 6.65 & -4.00 &   0 & 0.00 & 0.00 & AndVI &  & Local Group Sample \\ 
  98 & 2.65 & -3.00 &   0 & 0.00 & 0.00 & TucanaV &  & Local Group Sample \\ 
  99 & 4.06 & -3.00 &   0 & 0.00 & 0.00 & UrsaMajorI &  & Local Group Sample \\ 
  100 & 3.78 & -3.00 &   0 & 0.00 & 0.00 & UrsaMajorI &  & Local Group Sample \\ 
  101 & 6.54 & 10.00 &   1 & 1.00 & 5.03 & D634-03 &  & Georgiev Sample \\ 
  102 & 7.80 & 10.00 &   1 & 1.00 & 4.85 & DDO52 &  & Georgiev Sample \\ 
  104 & 6.99 & 10.00 &   1 & 1.00 & 4.61 & ESO121-20 &  & Georgiev Sample \\ 
  105 & 8.83 & 5.00 &   1 & 3.00 & 5.62 & ESO137-18 &  & Georgiev Sample \\ 
  106 & 8.30 & 8.90 &   1 & 3.00 & 4.55 & ESO154-023 &  & Georgiev Sample \\ 
  107 & 8.36 & 9.70 &   1 & 2.00 & 5.99 & ESO223-09 &  & Georgiev Sample \\ 
  108 & 8.48 & -2.20 &   1 & 2.00 & 0.00 & ESO269-58 &  & Georgiev Sample \\ 
  109 & 7.48 & -5.00 &   1 & 1.00 & 5.44 & ESO269-66 &  & Georgiev Sample \\ 
  110 & 9.18 & 6.60 &   1 & 7.00 & 5.95 & ESO274-01 &  & Georgiev Sample \\ 
  111 & 6.48 & 10.00 &   1 & 1.00 & 4.44 & ESO349-031 &  & Georgiev Sample \\ 
  112 & 7.73 & 9.80 &   1 & 1.00 & 4.36 & ESO381-20 &  & Georgiev Sample \\ 
  113 & 7.89 & -5.00 &   1 & 1.00 & 4.64 & ESO384-016 &  & Georgiev Sample \\ 
  114 & 8.15 & 8.40 &   1 & 3.00 & 5.12 & IC1959 &  & Georgiev Sample \\ 
  115 & 6.38 & -3.00 &   1 & 1.00 & 4.91 & IKN &  & Georgiev Sample \\ 
  116 & 6.72 & 10.00 &   1 & 1.00 & 4.32 & KK16 &  & Georgiev Sample \\ 
  117 & 6.00 & 10.00 &   1 & 1.00 & 4.04 & KK17 &  & Georgiev Sample \\ 
  118 & 6.98 & 10.00 &   1 & 1.00 & 4.48 & KK197 &  & Georgiev Sample \\ 
  120 & 5.85 & 10.00 &   1 & 2.00 & 4.78 & KK27 &  & Georgiev Sample \\ 
  123 & 8.07 & 8.70 &   1 & 2.00 & 4.67 & NGC1311 &  & Georgiev Sample \\ 
  124 & 9.37 & 6.90 &   1 & 24.00 & 6.58 & NGC247 &  & Georgiev Sample \\ 
  126 & 9.24 & 5.00 &   1 & 15.00 & 6.42 & NGC4605 &  & Georgiev Sample \\ 
  127 & 8.19 & 10.00 &   1 & 1.00 & 4.77 & NGC5237 &  & Georgiev Sample \\ 
  128 & 8.93 & 7.80 &   1 & 2.00 & 4.60 & NGC784 &  & Georgiev Sample \\ 
  129 & 8.10 & 7.50 &   1 & 1.00 & 5.17 & UGC1281 &  & Georgiev Sample \\ 
  130 & 7.97 & 9.90 &   1 & 3.00 & 5.81 & UGC3755 &  & Georgiev Sample \\ 
  132 & 7.93 & 9.90 &   1 & 4.00 & 5.08 & UGC4115 &  & Georgiev Sample \\ 
  134 & 8.24 & -3.00 &   1 & 8.00 & 5.67 & UGC7369 &  & Georgiev Sample \\ 
  135 & 7.21 & 9.90 &   1 & 1.00 & 6.34 & UGC8638 &  & Georgiev Sample \\ 
  136 & 7.03 & 9.80 &   1 & 1.00 & 4.12 & UGC8760 &  & Georgiev Sample \\ 
  137 & 8.22 & 9.90 &   1 & 1.00 & 6.67 & UGCA86 &  & Georgiev Sample \\ 
  138 & 7.65 & 10.00 &   1 & 1.00 & 5.42 & UGCA92 &  & Georgiev Sample \\ 
  121 & 7.60 & 10.00 &   1 & 1.00 & 4.37 & KKH77 &  & Georgiev Sample \\ 
  139 & 9.21 & 9.10 &   0 & 0.00 & 0.00 & LMC &  & Georgiev Sample \\ 
  140 & 8.57 & 8.90 &   0 & 0.00 & 0.00 & SMC &  & Georgiev Sample \\ 
  141 & 9.30 & 9.90 &   0 & 0.00 & 0.00 & NGC1427A &  & Georgiev Sample \\ 
  103 & 7.71 & 10.00 &   0 & 0.00 & 0.00 & ESO059-01 &  & Georgiev Sample \\ 
  119 & 6.99 & 10.00 &   0 & 0.00 & 0.00 & KK246 &  & Georgiev Sample \\ 
  122 & 6.23 & -3.00 &   0 & 0.00 & 0.00 & KKS55 &  & Georgiev Sample \\ 
  125 & 7.28 & 9.90 &   0 & 0.00 & 0.00 & NGC4163 &  & Georgiev Sample \\ 
  131 & 7.90 & 9.80 &   0 & 0.00 & 0.00 & UGC3974 &  & Georgiev Sample \\ 
  133 & 7.51 & 9.20 &   0 & 0.00 & 0.00 & UGC685 &  & Georgiev Sample \\ 
  301 & 9.55 & -5.00 &   1 & 1.00 & 6.69 & VCC0009 &  & Virgo Cluster Survey \\ 
  302 & 8.82 & -1.00 &   1 & 1.00 & 6.54 & VCC0021 &  & Virgo Cluster Survey \\ 
  303 & 8.69 & -5.00 &   1 & 1.00 & 5.55 & VCC0033 &  & Virgo Cluster Survey \\ 
  304 & 9.33 & -2.00 &   1 & 1.00 & 6.58 & VCC0140 &  & Virgo Cluster Survey \\ 
  305 & 8.80 & -5.00 &   1 & 1.00 & 6.43 & VCC0200 &  & Virgo Cluster Survey \\ 
  306 & 8.56 & -5.00 &   1 & 1.00 & 6.65 & VCC0230 &  & Virgo Cluster Survey \\ 
  307 & 10.15 & -2.00 &   1 & 1.00 & 7.35 & VCC0355 &  & Virgo Cluster Survey \\ 
  308 & 10.39 & -2.00 &   1 & 1.00 & 7.65 & VCC0369 &  & Virgo Cluster Survey \\ 
  309 & 9.12 & -2.00 &   1 & 1.00 & 6.89 & VCC0437 &  & Virgo Cluster Survey \\ 
  310 & 8.66 & -5.00 &   1 & 1.00 & 4.98 & VCC0538 &  & Virgo Cluster Survey \\ 
  311 & 9.07 & -2.00 &   1 & 1.00 & 6.51 & VCC0543 &  & Virgo Cluster Survey \\ 
  312 & 8.99 & 0.00 &   1 & 1.00 & 6.28 & VCC0571 &  & Virgo Cluster Survey \\ 
  313 & 9.70 & -5.00 &   1 & 1.00 & 6.56 & VCC0575 &  & Virgo Cluster Survey \\ 
  314 & 9.92 & 10.00 &   1 & 1.00 & 6.91 & VCC0654 &  & Virgo Cluster Survey \\ 
  315 & 10.36 & -2.00 &   1 & 1.00 & 7.68 & VCC0685 &  & Virgo Cluster Survey \\ 
  316 & 9.74 & -2.00 &   1 & 1.00 & 7.38 & VCC0698 &  & Virgo Cluster Survey \\ 
  317 & 11.24 & -5.00 &   1 & 1.00 & 9.03 & VCC0731 &  & Virgo Cluster Survey \\ 
  318 & 8.88 & 0.00 &   1 & 1.00 & 6.19 & VCC0751 &  & Virgo Cluster Survey \\ 
  319 & 10.51 & -2.00 &   1 & 1.00 & 7.71 & VCC0759 &  & Virgo Cluster Survey \\ 
  320 & 11.22 & -5.00 &   1 & 1.00 & 9.15 & VCC0763 &  & Virgo Cluster Survey \\ 
  321 & 10.06 & -2.00 &   1 & 1.00 & 7.22 & VCC0778 &  & Virgo Cluster Survey \\ 
  322 & 10.01 & -2.00 &   1 & 1.00 & 7.04 & VCC0784 &  & Virgo Cluster Survey \\ 
  323 & 11.15 & -2.00 &   1 & 1.00 & 8.56 & VCC0798 &  & Virgo Cluster Survey \\ 
  324 & 9.98 & -5.00 &   1 & 1.00 & 7.18 & VCC0828 &  & Virgo Cluster Survey \\ 
  325 & 9.14 & -5.00 &   1 & 1.00 & 6.89 & VCC0856 &  & Virgo Cluster Survey \\ 
  326 & 11.18 & -5.00 &   1 & 1.00 & 8.97 & VCC0881 &  & Virgo Cluster Survey \\ 
  327 & 10.27 & -2.00 &   1 & 1.00 & 7.24 & VCC0944 &  & Virgo Cluster Survey \\ 
  328 & 10.14 & -5.00 &   1 & 1.00 & 7.51 & VCC1025 &  & Virgo Cluster Survey \\ 
  329 & 10.58 & -2.00 &   1 & 1.00 & 7.94 & VCC1030 &  & Virgo Cluster Survey \\ 
  330 & 8.93 & 0.00 &   1 & 1.00 & 6.14 & VCC1049 &  & Virgo Cluster Survey \\ 
  331 & 10.57 & -2.00 &   1 & 1.00 & 7.66 & VCC1062 &  & Virgo Cluster Survey \\ 
  332 & 8.61 & -5.00 &   1 & 1.00 & 6.44 & VCC1075 &  & Virgo Cluster Survey \\ 
  333 & 9.23 & -5.00 &   1 & 1.00 & 7.09 & VCC1087 &  & Virgo Cluster Survey \\ 
  334 & 9.89 & -2.00 &   1 & 1.00 & 7.05 & VCC1125 &  & Virgo Cluster Survey \\ 
  335 & 9.84 & -5.00 &   1 & 1.00 & 7.19 & VCC1146 &  & Virgo Cluster Survey \\ 
  336 & 10.66 & -2.00 &   1 & 1.00 & 7.76 & VCC1154 &  & Virgo Cluster Survey \\ 
  337 & 9.70 & 3.00 &   1 & 1.00 & 6.71 & VCC1178 &  & Virgo Cluster Survey \\ 
  338 & 8.51 & -5.00 &   1 & 1.00 & 6.37 & VCC1185 &  & Virgo Cluster Survey \\ 
  339 & 9.34 & -5.00 &   1 & 1.00 & 7.19 & VCC1192 &  & Virgo Cluster Survey \\ 
  340 & 8.63 & -5.00 &   1 & 1.00 & 6.37 & VCC1199 &  & Virgo Cluster Survey \\ 
  341 & 11.45 & -5.00 &   1 & 1.00 & 9.39 & VCC1226 &  & Virgo Cluster Survey \\ 
  342 & 10.65 & -5.00 &   1 & 1.00 & 8.00 & VCC1231 &  & Virgo Cluster Survey \\ 
  343 & 10.05 & -2.00 &   1 & 1.00 & 7.42 & VCC1242 &  & Virgo Cluster Survey \\ 
  344 & 9.82 & -2.00 &   1 & 1.00 & 6.64 & VCC1250 &  & Virgo Cluster Survey \\ 
  345 & 9.66 & -5.00 &   1 & 1.00 & 6.91 & VCC1261 &  & Virgo Cluster Survey \\ 
  346 & 10.23 & -5.00 &   1 & 1.00 & 7.13 & VCC1279 &  & Virgo Cluster Survey \\ 
  347 & 9.74 & -2.00 &   1 & 1.00 & 7.09 & VCC1283 &  & Virgo Cluster Survey \\ 
  348 & 9.52 & -5.00 &   1 & 1.00 & 5.87 & VCC1297 &  & Virgo Cluster Survey \\ 
  349 & 9.86 & 0.00 &   1 & 1.00 & 7.18 & VCC1303 &  & Virgo Cluster Survey \\ 
  350 & 11.31 & -5.00 &   1 & 1.00 & 9.65 & VCC1316 &  & Virgo Cluster Survey \\ 
  351 & 9.76 & -5.00 &   1 & 1.00 & 6.82 & VCC1321 &  & Virgo Cluster Survey \\ 
  352 & 9.81 & -5.00 &   1 & 1.00 & 6.35 & VCC1327 &  & Virgo Cluster Survey \\ 
  353 & 8.34 & -5.00 &   1 & 1.00 & 6.29 & VCC1355 &  & Virgo Cluster Survey \\ 
  354 & 8.73 & -5.00 &   1 & 1.00 & 6.91 & VCC1407 &  & Virgo Cluster Survey \\ 
  355 & 9.28 & -5.00 &   1 & 1.00 & 6.67 & VCC1422 &  & Virgo Cluster Survey \\ 
  356 & 9.13 & -5.00 &   1 & 1.00 & 7.03 & VCC1431 &  & Virgo Cluster Survey \\ 
  357 & 8.93 & -5.00 &   1 & 1.00 & 6.65 & VCC1440 &  & Virgo Cluster Survey \\ 
  358 & 9.66 & -2.00 &   1 & 1.00 & 7.22 & VCC1475 &  & Virgo Cluster Survey \\ 
  359 & 9.66 & -3.00 &   1 & 1.00 & 7.22 & VCC1488 &  & Virgo Cluster Survey \\ 
  360 & 8.57 & -5.00 &   1 & 1.00 & 6.24 & VCC1489 &  & Virgo Cluster Survey \\ 
  361 & 8.55 & -5.00 &   1 & 1.00 & 6.49 & VCC1499 &  & Virgo Cluster Survey \\ 
  362 & 8.83 & -2.00 &   1 & 1.00 & 5.87 & VCC1512 &  & Virgo Cluster Survey \\ 
  363 & 8.83 & -3.00 &   1 & 1.00 & 5.87 & VCC1528 &  & Virgo Cluster Survey \\ 
  364 & 10.98 & -2.00 &   1 & 1.00 & 8.06 & VCC1535 &  & Virgo Cluster Survey \\ 
  365 & 9.92 & -2.00 &   1 & 1.00 & 6.83 & VCC1537 &  & Virgo Cluster Survey \\ 
  366 & 8.75 & -5.00 &   1 & 1.00 & 6.68 & VCC1539 &  & Virgo Cluster Survey \\ 
  367 & 8.72 & -5.00 &   1 & 1.00 & 6.96 & VCC1545 &  & Virgo Cluster Survey \\ 
  368 & 10.00 & -2.00 &   1 & 1.00 & 7.27 & VCC1619 &  & Virgo Cluster Survey \\ 
  369 & 9.03 & -5.00 &   1 & 1.00 & 5.76 & VCC1627 &  & Virgo Cluster Survey \\ 
  370 & 9.98 & -5.00 &   1 & 1.00 & 7.01 & VCC1630 &  & Virgo Cluster Survey \\ 
  371 & 10.73 & -5.00 &   1 & 1.00 & 8.44 & VCC1632 &  & Virgo Cluster Survey \\ 
  372 & 8.65 & -5.00 &   1 & 1.00 & 6.19 & VCC1661 &  & Virgo Cluster Survey \\ 
  373 & 10.34 & -5.00 &   1 & 1.00 & 7.71 & VCC1664 &  & Virgo Cluster Survey \\ 
  374 & 10.50 & -2.00 &   1 & 1.00 & 7.54 & VCC1692 &  & Virgo Cluster Survey \\ 
  375 & 8.90 & 0.00 &   1 & 1.00 & 6.41 & VCC1695 &  & Virgo Cluster Survey \\ 
  376 & 10.15 & -2.00 &   1 & 1.00 & 7.15 & VCC1720 &  & Virgo Cluster Survey \\ 
  377 & 8.55 & -5.00 &   1 & 1.00 & 6.19 & VCC1743 &  & Virgo Cluster Survey \\ 
  378 & 8.37 & 0.00 &   1 & 1.00 & 5.55 & VCC1779 &  & Virgo Cluster Survey \\ 
  379 & 8.33 & -5.00 &   1 & 1.00 & 5.84 & VCC1826 &  & Virgo Cluster Survey \\ 
  380 & 8.65 & 5.00 &   1 & 1.00 & 6.53 & VCC1828 &  & Virgo Cluster Survey \\ 
  381 & 9.07 & -5.00 &   1 & 1.00 & 6.49 & VCC1833 &  & Virgo Cluster Survey \\ 
  382 & 8.98 & 10.00 &   1 & 1.00 & 6.25 & VCC1857 &  & Virgo Cluster Survey \\ 
  383 & 9.19 & -5.00 &   1 & 1.00 & 6.83 & VCC1861 &  & Virgo Cluster Survey \\ 
  384 & 9.25 & -5.00 &   1 & 1.00 & 6.26 & VCC1871 &  & Virgo Cluster Survey \\ 
  385 & 10.32 & -2.00 &   1 & 1.00 & 7.36 & VCC1883 &  & Virgo Cluster Survey \\ 
  386 & 8.83 & -5.00 &   1 & 1.00 & 5.79 & VCC1886 &  & Virgo Cluster Survey \\ 
  387 & 8.71 & -5.00 &   1 & 1.00 & 6.01 & VCC1895 &  & Virgo Cluster Survey \\ 
  388 & 10.80 & -5.00 &   1 & 1.00 & 8.36 & VCC1903 &  & Virgo Cluster Survey \\ 
  389 & 9.27 & -5.00 &   1 & 1.00 & 6.94 & VCC1910 &  & Virgo Cluster Survey \\ 
  390 & 9.95 & -2.00 &   1 & 1.00 & 7.23 & VCC1913 &  & Virgo Cluster Survey \\ 
  391 & 10.33 & -2.00 &   1 & 1.00 & 7.16 & VCC1938 &  & Virgo Cluster Survey \\ 
  392 & 8.75 & -5.00 &   1 & 1.00 & 5.59 & VCC1948 &  & Virgo Cluster Survey \\ 
  393 & 11.31 & -5.00 &   1 & 1.00 & 9.13 & VCC1978 &  & Virgo Cluster Survey \\ 
  394 & 8.55 & -5.00 &   1 & 1.00 & 5.59 & VCC1993 &  & Virgo Cluster Survey \\ 
  395 & 10.22 & -5.00 &   1 & 1.00 & 7.68 & VCC2000 &  & Virgo Cluster Survey \\ 
  396 & 9.10 & -5.00 &   1 & 1.00 & 6.63 & VCC2019 &  & Virgo Cluster Survey \\ 
  397 & 9.19 & -5.00 &   1 & 1.00 & 6.51 & VCC2048 &  & Virgo Cluster Survey \\ 
  398 & 8.54 & -5.00 &   1 & 1.00 & 6.17 & VCC2050 &  & Virgo Cluster Survey \\ 
  399 & 10.55 & -2.00 &   1 & 1.00 & 7.45 & VCC2092 &  & Virgo Cluster Survey \\ 
  400 & 10.93 & -2.00 &   1 & 1.00 & 7.86 & VCC2095 &  & Virgo Cluster Survey \\ 
  401 & 11.01 & 3.00 &   1 & 1.00 & 8.28 & VCC 167 &  & Virgo Cluster Survey \\ 
  402 & 8.72 & -5.00 &   1 & 1.00 & 6.20 & VCC 158 &  & Virgo Cluster Survey \\ 
  403 & 7.77 & -5.00 &   1 & 1.00 & 6.04 & VCC 240 &  & Virgo Cluster Survey \\ 
  404 & 9.49 & -5.00 &   1 & 1.00 & 6.16 & VCC 308 &  & Virgo Cluster Survey \\ 
  405 & 8.68 & -5.00 &   1 & 1.00 & 6.44 & VCC 452 &  & Virgo Cluster Survey \\ 
  406 & 8.28 & -5.00 &   1 & 1.00 & 5.61 & VCC 503 &  & Virgo Cluster Survey \\ 
  407 & 7.72 & -5.00 &   1 & 1.00 & 5.72 & VCC 529 &  & Virgo Cluster Survey \\ 
  408 & 7.49 & -5.00 &   1 & 1.00 & 5.83 & VCC 646 &  & Virgo Cluster Survey \\ 
  409 & 8.52 & -5.00 &   1 & 1.00 & 6.38 & VCC 747 &  & Virgo Cluster Survey \\ 
  410 & 8.87 & -5.00 &   1 & 1.00 & 6.46 & VCC 871 &  & Virgo Cluster Survey \\ 
  411 & 7.92 & -5.00 &   1 & 1.00 & 5.84 & VCC 896 &  & Virgo Cluster Survey \\ 
  412 & 8.97 & -5.00 &   1 & 1.00 & 7.02 & VCC 940 &  & Virgo Cluster Survey \\ 
  413 & 8.96 & -5.00 &   1 & 1.00 & 6.58 & VCC 949 &  & Virgo Cluster Survey \\ 
  414 & 8.60 & -5.00 &   1 & 1.00 & 6.39 & VCC 965 &  & Virgo Cluster Survey \\ 
  415 & 8.57 & -5.00 &   1 & 1.00 & 5.73 & VCC 992 &  & Virgo Cluster Survey \\ 
  416 & 9.27 & -5.00 &   1 & 1.00 & 6.55 & VCC1073 &  & Virgo Cluster Survey \\ 
  417 & 7.35 & -5.00 &   1 & 1.00 & 5.35 & VCC1077 &  & Virgo Cluster Survey \\ 
  418 & 8.81 & -5.00 &   1 & 1.00 & 6.10 & VCC1104 &  & Virgo Cluster Survey \\ 
  419 & 8.55 & -5.00 &   1 & 1.00 & 5.85 & VCC1105 &  & Virgo Cluster Survey \\ 
  420 & 8.96 & -5.00 &   1 & 1.00 & 6.62 & VCC1107 &  & Virgo Cluster Survey \\ 
  421 & 8.73 & -5.00 &   1 & 1.00 & 6.33 & VCC1167 &  & Virgo Cluster Survey \\ 
  422 & 7.48 & -5.00 &   1 & 1.00 & 5.98 & VCC1252 &  & Virgo Cluster Survey \\ 
  423 & 8.88 & -5.00 &   1 & 1.00 & 6.63 & VCC1254 &  & Virgo Cluster Survey \\ 
  424 & 7.62 & -5.00 &   1 & 1.00 & 5.57 & VCC1272 &  & Virgo Cluster Survey \\ 
  425 & 8.59 & -5.00 &   1 & 1.00 & 6.13 & VCC1308 &  & Virgo Cluster Survey \\ 
  426 & 8.73 & -5.00 &   1 & 1.00 & 6.49 & VCC1311 &  & Virgo Cluster Survey \\ 
  427 & 8.29 & -5.00 &   1 & 1.00 & 6.19 & VCC1333 &  & Virgo Cluster Survey \\ 
  428 & 7.40 & -5.00 &   1 & 1.00 & 6.19 & VCC1363 &  & Virgo Cluster Survey \\ 
  429 & 9.20 & -5.00 &   1 & 1.00 & 6.67 & VCC1386 &  & Virgo Cluster Survey \\ 
  430 & 8.73 & -5.00 &   1 & 1.00 & 5.95 & VCC1497 &  & Virgo Cluster Survey \\ 
  431 & 8.96 & -5.00 &   1 & 1.00 & 5.53 & VCC1514 &  & Virgo Cluster Survey \\ 
  432 & 7.68 & -5.00 &   1 & 1.00 & 5.99 & VCC1530 &  & Virgo Cluster Survey \\ 
  433 & 8.69 & -5.00 &   1 & 1.00 & 6.35 & VCC1577 &  & Virgo Cluster Survey \\ 
  434 & 9.03 & -2.00 &   1 & 1.00 & 6.65 & VCC1614 &  & Virgo Cluster Survey \\ 
  435 & 7.61 & -5.00 &   1 & 1.00 & 6.19 & VCC1714 &  & Virgo Cluster Survey \\ 
  436 & 9.05 & -5.00 &   1 & 1.00 & 6.64 & VCC1876 &  & Virgo Cluster Survey \\ 
   \hline
\end{tabular}
\end{table}


==> coeff_table.tex <==

% Table created by stargazer v.5.2.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Fri, Dec 04, 2020 - 01:42:12 PM
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{tab:solutions} 
\begin{tabular}{@{\extracolsep{5pt}}lccccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{7}{c}{\textit{Dependent variable:}} \\ 
\cline{2-8} 
\\[-1.8ex] & \multicolumn{7}{c}{hasGC} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7)\\ 
\hline \\[-1.8ex] 
 log10Mstar & 1.838$^{***}$ & 1.881$^{***}$ & 1.310$^{***}$ & 1.224$^{***}$ &  & 1.722$^{***}$ & 1.735$^{***}$ \\ 
  & (0.439) & (0.460) & (0.221) & (0.237) &  & (0.218) & (0.220) \\ 
  & & & & & & & \\ 
 Type &  & $-$0.023 &  & 0.037 &  &  & $-$0.043 \\ 
  &  & (0.068) &  & (0.042) &  &  & (0.037) \\ 
  & & & & & & & \\ 
 SampleGeorgiev sample &  &  &  &  & 1.289$^{**}$ &  &  \\ 
  &  &  &  &  & (0.556) &  &  \\ 
  & & & & & & & \\ 
 log10MstarCentered &  &  &  &  & 1.105$^{***}$ &  &  \\ 
  &  &  &  &  & (0.227) &  &  \\ 
  & & & & & & & \\ 
 Constant & $-$13.282$^{***}$ & $-$13.545$^{***}$ & $-$9.212$^{***}$ & $-$8.756$^{***}$ & $-$0.609$^{*}$ & $-$11.698$^{***}$ & $-$11.714$^{***}$ \\ 
  & (3.014) & (3.124) & (1.539) & (1.608) & (0.350) & (1.570) & (1.563) \\ 
  & & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 99 & 99 & 140 & 140 & 140 & 276 & 276 \\ 
Log Likelihood & $-$19.024 & $-$18.966 & $-$49.622 & $-$49.226 & $-$46.936 & $-$56.686 & $-$55.993 \\ 
Akaike Inf. Crit. & 42.048 & 43.933 & 103.243 & 104.452 & 99.873 & 117.372 & 117.985 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{7}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 

